Weakly supervised cross-domain alignment with optimal transport

Cross-domain alignment between image objects and text sequences is key to many visual-language tasks, and it poses a fundamental challenge to both computer vision and natural language processing. This paper investigates a novel approach for the identification and optimization of fine-grained semantic similarities between image and text entities, under a weakly-supervised setup, improving performance over state-of-the-art solutions. Our method builds upon recent advances in optimal transport (OT) to resolve the cross-domain matching problem in a principled manner. Formulated as a drop-in regularizer, the proposed OT solution can be efficiently computed and used in combination with other existing approaches. We present empirical evidence to demonstrate the effectiveness of our approach, showing how it enables simpler model architectures to outperform or be comparable with more sophisticated designs on a range of vision-language tasks.

==> alg/algorithm_ot.tex <==
% % \begin{wrapfigure}[12]{R}{0.45\textwidth}
% % \begin{minipage}{0.5\textwidth}
% % \vspace{-12mm}

% % \begin{minipage}{1.0\textwidth}
% % \begin{wrapfigure}[12]{R}{0.45\textwidth}
% \vspace{-2em}
% \begin{algorithm}[H]
% \footnotesize
% \caption{\footnotesize IPOT algorithm}
% \label{alg:ipot}
% \begin{algorithmic}[1]
% \State {\bfseries Input:} \footnotesize{\footnotesize{Feature vectors 
% % $\{\xv_i\}=\{\Smat_i\}_1^n$ and $\{\yv_i\}=\{\Smat'_j\}_1^m$, generalized stepsize $1/\beta$
%  $\Smat=\{\zv_i\}_1^n$, $\Smat'=\{\zv'_j\}_1^m$ $\,\,\,\,$ and generalized stepsize $1/\beta$, 
% }}

% \State $\boldsymbol{\sigma}=\frac{1}{m}\mathbf{1_m}$, $\Tmat^{(1)} = \mathbf{1_n} \mathbf{1_m}^\top$
% \State $\Cmat_{ij} = c(\zv_i, \zv'_j)$, $\Amat_{ij} = {\rm e}^{-\frac{\Cmat_{ij}}{\beta}}$
% \For{$t=1,2,3,\ldots,N$} \footnotesize{// $N$ is a hyperparameter}
%     \State $\Qmat = \Amat \odot \Tmat^{(t)}$ \footnotesize{// $\odot$ is Hadamard product}
%     \For{$k=1,\ldots K$} \footnotesize{// $K=1$ in practice}
%         \State $\boldsymbol{\delta} = \frac{1}{n\Qmat{\boldsymbol{\sigma}}}$, $\boldsymbol{\sigma} = \frac{1}{m\Qmat^\top\boldsymbol{\delta}}$
%     \EndFor
%     \State $\Tmat^{(t+1)} = \text{diag}(\boldsymbol{\delta})\Qmat\text{diag}(\boldsymbol{\sigma})$
% \EndFor
% % \State $\Lcal_{\text{ot}} = \langle \Tmat, \Cmat \rangle$
% \State \textbf{Return} $\langle \Tmat, \Cmat \rangle$
% \end{algorithmic}
% \end{algorithm}
% % \end{minipage}
% % \end{wrapfigure}

% \begin{wrapfigure}[9]{r}{0.45\textwidth}
    \begin{minipage}{0.6\textwidth}
    % \vspace{-50pt}
      \begin{algorithm}[H]
       \caption{IPOT($\mathbf{E}, \Vmat$, $\beta$)}
	 \begin{algorithmic}
            \STATE \textbf{Input:} $\mathbf{E}=\{\ev_i\}_1^M, \Vmat=\{\vv_i\}_1^K$, hyper-parameter $\beta$
            \STATE calcuate cost matrix $\Cmat = C(\Vmat,\mathbf{E})$
        	\STATE $\bm{b}\leftarrow \frac{1}{m}\pmb{1}_m$, $\bm{\Tmat}^{(1)} \leftarrow  \pmb{11}^T$
        	\STATE $\Gmat_{ij}\leftarrow \exp(-\frac{\bm{C}_{ij}}{\beta})$
        	\FOR {$t=1,2,3,..., N$}
        	\STATE $\bm{Q} \leftarrow  \bm{G}\odot \bm{\Tmat}^{(t)}$
        	\STATE \textbf{for} {$l=1,2,3,...,L$} \textbf{do}$\quad$ // Usually set $L=1$
        	\STATE \quad $\bm{a}\leftarrow \frac{1}{K\bm{Qb}}$, $\bm{b}\leftarrow \frac{1}{M\bm{Q}^T \bm{a}}$
        	\STATE \textbf{end for}
        	\STATE $\bm{\Tmat}^{(t+1)} \leftarrow  \text{diag}(\bm{a}) \bm{Q} \text{diag}(\bm{b})$
        	\ENDFOR
        \end{algorithmic} \label{alg:ipot}
      \end{algorithm}
      \vspace{-0pt}
    \end{minipage}
%   \end{wrapfigure}

==> mlVecMat.tex <==
%\usepackage{hyperref}
\usepackage{url}
%\documentstyle[nips14submit_09,times,art10]{article} % For LaTeX 2.09

\newcommand{\RN}[1]{%
	\textup{\lowercase\expandafter{\it \romannumeral#1}}%
}

\usepackage{amsmath}
%\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{wrapfig}
\usepackage{bm}
\usepackage{subcaption}
\usepackage{psfrag}
\usepackage{epstopdf}
\usepackage{multirow}
% \usepackage{fullpage}
\usepackage{mathtools} 

\usepackage{verbatim}

\usepackage{color}
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,snakes,automata,backgrounds,fit,petri}
\usepackage{adjustbox}


% For algorithms
\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage[lined,boxed,commentsnumbered,ruled,algo2e]{algorithm2e}

\let\oldnorm\norm   % <-- Store original \norm as \oldnorm
\let\norm\undefined % <-- "Undefine" \norm
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

\def\Dir{\textsf{Dir}} %normal distribution symbol
\def\Bern{\textsf{Ber}} %Bernoulii distribution symbol
\def\Pois{\textsf{Pois}} %poisson distribution symbol
\def\Std{\textsf{Std}} %Standard deviation function symbol
\def\Var{\textsf{Var}} %Variance function symbol
\def\Cor{\textsf{Cor}} %correlation function symbol
\def\Cov{\textsf{Cov}} %covariance function symbol
\def\Gal{\textsf{Gamma}} %covariance function symbol

\newcommand{\ie}[0]{\emph{i.e., }}
\newcommand{\ea}[0]{\emph{et al. }}
\newcommand{\eg}[0]{\emph{e.g., }}
\newcommand{\cf}[0]{\emph{cf. }}
\newcommand{\etc}[0]{\emph{etc.}}

\newcommand{\zerov}[0]{\ensuremath{{\bf 0}}\xspace}
\newcommand{\onev}[0]{\ensuremath{{\bf 1}}\xspace}

\newcommand{\beq}{\vspace{0mm}\begin{equation}}
\newcommand{\eeq}{\vspace{0mm}\end{equation}}
\newcommand{\beqs}{\vspace{0mm}\begin{eqnarray}}
\newcommand{\eeqs}{\vspace{0mm}\end{eqnarray}}
\newcommand{\barr}{\begin{array}}
\newcommand{\earr}{\end{array}}

\newcommand{\Amat}[0]{{{\bf A}}}
\newcommand{\Bmat}{{\bf B}}
\newcommand{\Cmat}{{\bf C}}
\newcommand{\Dmat}{{\bf D}}
\newcommand{\Emat}[0]{{{\bf E}}}
\newcommand{\Fmat}[0]{{{\bf F}}\xspace}
\newcommand{\Gmat}{{\bf G}}
\newcommand{\Hmat}{{\bf H}}
\newcommand{\Imat}{{\bf I}}
\newcommand{\Jmat}[0]{{{\bf J}}\xspace}
\newcommand{\Kmat}[0]{{{\bf K}}\xspace}
\newcommand{\Lmat}[0]{{{\bf L}}}
%\newcommand{\Mmat}[0]{{{\bf M}}\xspace}
\newcommand{\Mmat}{{\bf M}}
\newcommand{\Nmat}[0]{{{\bf N}}\xspace}
\newcommand{\Omat}[0]{{{\bf O}}}
\newcommand{\Pmat}{{\bf P}}
\newcommand{\Qmat}[0]{{{\bf Q}}\xspace}
\newcommand{\Rmat}[0]{{{\bf R}}}
\newcommand{\Smat}[0]{{{\bf S}}}
\newcommand{\Tmat}[0]{{{\bf T}}}
\newcommand{\Umat}[0]{{{\bf U}}}
\newcommand{\Vmat}[0]{{{\bf V}}}
\newcommand{\Wmat}[0]{{{\bf W}}}
\newcommand{\Xmat}[0]{{{\bf X}}}
\newcommand{\Ymat}{{\bf Y}}
%\newcommand{\Ymat}[0]{{{\bf Z}}}
\newcommand{\Zmat}{{\bf Z}}

\newcommand{\av}[0]{{\boldsymbol{a}}}
\newcommand{\bv}[0]{{\boldsymbol{b}}}
\newcommand{\cv}[0]{{\boldsymbol{c}}}
\newcommand{\dv}{\boldsymbol{d}}
\newcommand{\ev}[0]{{\boldsymbol{e}}\xspace}
\newcommand{\fv}[0]{{\boldsymbol{f}}\xspace}
\newcommand{\gv}[0]{{\boldsymbol{g}}}
\newcommand{\hv}[0]{{\boldsymbol{h}}}
\newcommand{\iv}[0]{{\boldsymbol{i}}\xspace}
\newcommand{\jv}[0]{{\boldsymbol{j}}\xspace}
\newcommand{\kv}[0]{{\boldsymbol{k}}\xspace}
\newcommand{\lv}[0]{{\boldsymbol{l}}}
\newcommand{\mv}[0]{{\boldsymbol{m}}}
\newcommand{\nv}[0]{{\boldsymbol{n}}\xspace}
\newcommand{\ov}[0]{{\boldsymbol{o}}\xspace}
\newcommand{\pv}[0]{{\boldsymbol{p}}}
\newcommand{\qv}[0]{{\boldsymbol{q}}\xspace}
\newcommand{\rv}{\boldsymbol{r}}
\newcommand{\sv}[0]{{\boldsymbol{s}}}
\newcommand{\tv}[0]{{\boldsymbol{t}}\xspace}
\newcommand{\uv}{\boldsymbol{u}}
\newcommand{\vv}{\boldsymbol{v}}
\newcommand{\wv}{\boldsymbol{w}}
\newcommand{\xv}{\boldsymbol{x}}
\newcommand{\yv}{\boldsymbol{y}}
\newcommand{\cv}{\boldsymbol{c}}
\newcommand{\zv}{\boldsymbol{z}}
\newcommand{\cdotv}{\boldsymbol{\cdot}}

\newcommand{\Gammamat}[0]{{\boldsymbol{\Gamma}}\xspace}
\newcommand{\Deltamat}[0]{{\boldsymbol{\Delta}}\xspace}
\newcommand{\Thetamat}{\boldsymbol{\Theta}}
\newcommand{\Betamat}{\boldsymbol{\Beta}}
\newcommand{\Lambdamat}{\boldsymbol{\Lambda}}
\newcommand{\Ximat}[0]{{\boldsymbol{\Xi}}\xspace}
\newcommand{\Pimat}[0]{{\boldsymbol{\Pi}}\xspace}
\newcommand{\Sigmamat}[0]{{\boldsymbol{\Sigma}}}
\newcommand{\Upsilonmat}[0]{{\boldsymbol{\Upsilon}}\xspace}
\newcommand{\Phimat}{\boldsymbol{\Phi}}
\newcommand{\Psimat}{\boldsymbol{\Psi}}
\newcommand{\Omegamat}[0]{{\boldsymbol{\Omega}}}

\newcommand{\alphav}{\boldsymbol{\alpha}}
\newcommand{\betav}[0]{{\boldsymbol{\beta}}}
\newcommand{\gammav}[0]{{\boldsymbol{\gamma}}\xspace}
\newcommand{\deltav}[0]{{\boldsymbol{\delta}}\xspace}
\newcommand{\epsilonv}{\boldsymbol{\epsilon}}
\newcommand{\zetav}{\boldsymbol{\zeta}}
\newcommand{\etav}[0]{{\boldsymbol{\eta}}\xspace}
\newcommand{\ellv}[0]{{\boldsymbol{\ell}}}
\newcommand{\thetav}{\boldsymbol{\theta}}
\newcommand{\iotav}[0]{{\boldsymbol{\iota}}}
\newcommand{\kappav}[0]{{\boldsymbol{\kappa}}\xspace}
\newcommand{\lambdav}[0]{{\boldsymbol{\lambda}}}
\newcommand{\muv}[0]{{\boldsymbol{\mu}}}
\newcommand{\nuv}[0]{{\boldsymbol{\nu}}}
\newcommand{\xiv}[0]{{\boldsymbol{\xi}}}
\newcommand{\omicronv}[0]{{\boldsymbol{\omicron}}\xspace}
\newcommand{\piv}{\boldsymbol{\pi}}
\newcommand{\rhov}[0]{{\boldsymbol{\rho}}\xspace}
\newcommand{\sigmav}[0]{{\boldsymbol{\sigma}}}
\newcommand{\tauv}[0]{{\boldsymbol{\tau}}\xspace}
\newcommand{\upsilonv}[0]{{\boldsymbol{\upsilon}}\xspace}
\newcommand{\phiv}{\boldsymbol{\phi}}
\newcommand{\chiv}[0]{{\boldsymbol{\chi}}\xspace}
\newcommand{\psiv}{\boldsymbol{\psi}}
\newcommand{\varthetav}{\boldsymbol{\vartheta}}
%\newcommand{\zetav}{\boldsymbol{\zeta}}
\newcommand{\omegav}[0]{{\boldsymbol{\omega}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Z}{\mathbb{Z}}

\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Hcal}{\mathcal{H}}

\newtheorem{theorem}{Theorem} %[section]
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}

\DeclareMathOperator{\CC}{\mathbb{C}} % Complex numbers
\DeclareMathOperator{\EE}{\mathbb{E}} % Expectation
\DeclareMathOperator{\KK}{\mathbb{K}} % Arbitrary field
\DeclareMathOperator{\MM}{\mathbb{M}} % Median
\DeclareMathOperator{\NN}{\mathbb{N}} % Natural numbers
\DeclareMathOperator{\PP}{\mathbb{P}} % Probability
\DeclareMathOperator{\QQ}{\mathbb{Q}} % Rationals
\DeclareMathOperator{\RR}{\mathbb{R}} % Real numbers
\DeclareMathOperator{\ZZ}{\mathbb{Z}} % Integers
\DeclareMathOperator{\Tr}{Tr}

\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi

\newenvironment{proof}[1][Proof]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{definition}[1][Definition]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

 \newcommand{\hlightP}[1]{%
 	\ooalign{\hss\makebox[0pt]{\fcolorbox{red!30}{green!10}{$#1$}}\hss\cr\phantom{$#1$}}%
 }
 
 \newcommand{\hlightC}[1]{%
 	\ooalign{\hss\makebox[0pt]{\fcolorbox{green!30}{red!40}{$#1$}}\hss\cr\phantom{$#1$}}%
 }


%\newcommand{\qed}{\nobreak \ifvmode \relax \else
%      \ifdim\lastskip<1.5em \hskip-\lastskip
%      \hskip1.5em plus0em minus0.5em \fi \nobreak
%      \vrule height0.75em width0.5em depth0.25em\fi}

==> removed_part.tex <==
%
%Relative to existing solutions, our OT-based CDA features the following highlights: $(\RN{1})$ OT tries to discover all possible alignments for each pair of image regions and descriptions. The pattern inferred by OT is more interpretable and principle. $(\RN{2})$ OT distance can be used as a new loss function which can provide a global view of how image and text is aligned. So that OT can be used as a complementary regularizer to fine-tune the matching model.
%Specifically, we represent image and text with set of vectors, then using OT to calculate the matching plan. In order to extract salient features from images, we follow the same setup as \cite{anderson2018bottom}, which is built upon faster R-CNN~\cite{ren2015faster}. To extract salient features from sentences, we use bi-directional GRU~\cite{schuster1997bidirectional, bahdanau2014neural} to better capture the important content information from the sentence, inspired by \cite{conneau2017supervised}.

%Comparing with these previous attention methods, our OT algorithm has these advantages: $(\RN{1})$ OT tries to discover all possible alignments for each pair of image regions and descriptions. The pattern inferred by OT is more interpretable and principle. $(\RN{2})$ OT distance can be used as a new loss function which can provide a global view of how image and text is aligned. So that OT can be used as a complementary regularizer to fine-tune the matching model.
%Specifically, we represent image and text with set of vectors, then using OT to calculate the matching plan. In order to extract salient features from images, we follow the same setup as \cite{anderson2018bottom}, which is built upon faster R-CNN~\cite{ren2015faster}. To extract salient features from sentences, we use bi-directional GRU~\cite{schuster1997bidirectional, bahdanau2014neural} to better capture the important content information from the sentence, inspired by \cite{conneau2017supervised}.

%Many works have explored the problem of matching image features and sentence features to a common semantic space for image-text matching. The first attempt is made by \cite{kiros2014unifying}, the authors propose to use convolutional neural networks to encode the images and LSTM to encode sentences. The model is trained with a hinge-base triplet ranking loss. \citep{VSE} improved \cite{kiros2014unifying} by adding hardest negatives in the triplet ranking loss. 
%\cite{karpathy2015deep} first proposed to consider the relationship between image regions and descriptions. They first compute the similarity matrix for all regions-words pairs with dot-product, then calculate the similarity score with sum or max aggregation function. 
%Recently, SCAN~\cite{SCAN} model is proposed to use stacked cross attention to connect corresponding region and text pairs. The framework of SCAN is a two steps attention model. Basically, it uses images to attend sentences to get attention scores and attended sentence vector in Step 1. Step 2, the importance of image region is evaluated by the similarity between the region and corresponding attended sentence vector. 
%In our model, we share the same motivation as SCAN, but we come up with an easy and principle way, optimal transport, to obtain the relevance between two domains.

% \rhg{why is this all in italics?}
% {\it 
% One core aspect leading to good performance in CDA tasks is that features from both domains need to be properly aligned.
% This is consistent with human behavior.
% As shown in Figure \ref{fig:intuition}, when humans generates descriptions for an image, they often reference certain regions of the image.
% Inferring the alignment between image regions and words is crucial since it may result in more interpretable image-to-text matching, thus further helpful at leveraging fine-grained cross-domain correspondence information.
%
% However, the image-to-text matching task is a ``weakly'' unsupervised task.
% Despite having paired data, the correspondence (labels) between image regions and words is not available \cite{harwath2018jointly}.
% Therefore, finding such alignment is very challenging: $i$) for images we need to simultaneously detect and characterize the interactions between different objects from image features; $ii$) for text sentences we need to obtain features about descriptions with the salient information which can indicate the relationship, position information, {\it etc};
% $iii$) features containing objective and salient information from different domains needs to be aligned properly without any labels.

% Consider the problem of matching phrases/words to image regions, which can be formulated as a bipartite matching problem as shown in the Figure \ref{fig:intuition}, and can be solved by the maximum network flow algorithm~\cite{edmonds1972theoretical, fredman1987fibonacci}.



% Image Representation
% To this end, $\Vmat$ is obtained from a pre-trained {\it faster R-CNN}~\cite{ren2015faster} (fR-CNN), which is a two-stage object detection model.
% % that first proposes regions and then summarizes them in terms of features (embeddings).
% fR-CNN first employs a region proposal network (RPN) to propose image regions.
% % Meanwhile, it predicts an {\it objectness} score \rhg{such as?} at each location, which quantifies model's confidence on whether a particular region contains or refers to an object of interest.
% The proposed regions are fed to an encoder network for feature extraction. In particular, fR-CNN leverages RoI pooling to construct fixed length feature vectors. The fixed length feature vector is then used for object classification.
% In \cite{anderson2018bottom} the score for a region is defined as the highest class detection probability for the region, quantifying the confidence of the model on whether a particular region contains or refers to an object of interest. We denote this score as {\it object} score.
% To ensure that fR-CNN captures a wide variety of concepts, it was pre-trained on a heavily annotated dataset.
% Specifically, the Visual Genome dataset~\citep{krishna2017visual}.
% In this study, we follow \citep{anderson2018bottom}, where they used a ResNet-101 \citep{he2016deepresidual} to obtain a $2048$-dimensional feature vectors denoted $\fv_k$ for each region $k$.
% Once pre-trained, the fR-CNN parameters are kept fixed.
% To project the image features into a feature space shared by sentence features (see below), we further apply a custom affine transformation to $\fv_k$:
% %
% \begin{equation}
%     \vv_k = \Wmat_v \fv_k + \bv_v,
% \end{equation}
% %
% where $\Wmat_v \in \R^{d \times 2048}$ and $\bv_v \in \R^d$ are affine learnable parameters.

==> table/Ablation_sm.tex <==
\begin{table*}[h!] \footnotesize
    \begin{center}
    % \begin{tabular}{lccccccc}
        \caption{Ablation study on Flickr30K. In the first section, we try to use adaptive features. In the second section, we compare the performance of different network architectures for text representations.}
        \label{table:ablation_sm}
            \centering
        \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
            \toprule
            % \noalign{\smallskip}
             & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{} \\
            Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & Rsum\\
            % \noalign{\smallskip}
            \hline
            \noalign{\smallskip}
            $\cos$ + OT, fixed & 67.4 & 90.3 & 94.9 & 48.2 & 76.7 & {84.8} &462.3 \\ 
            $\cos$ + OT, adaptive & 64.8 & 88.3 &94.5 & 45.9 & 74.5 & 83.5 &451.5 \\
            % \midrule
            % $\cos$, $\eta$=0.2  & 61.7 & 87.4 & 93.5 & 48.5 & 76.0 & 83.7 & 450.8 \\ 
            % $\cos$ + OT, $\eta$=0.2, $\lambda$=1 & 66.2 & 89.0 & 94.1 & 48.9 & 77.5 & {85.4} &461.1 \\ 
            % % \hline
            % $\cos$, $\eta$=0.12  & 63.1 &89.5 & 94.3 & {50.5} & 77.1 & 84.7&459.2 \\ 
            % $\cos$ + OT, $\eta$=0.12, $\lambda$=2 & {69.3} & {91.0} &{95.7} & 48.4 & {77.2} & 84.7 &{466.3} \\
            \midrule
            $\cos$+OT, bi-GRU &{67.9} &{91.0} &{94.9} &{49.8} &{77.5} &{85.2} &{466.3}\\
            $\cos$+OT, Transformer, 1 layer, 8 heads & 57.8 & 86.8 & 93.1 & 46.4 & 74.4 & {82.9} &441.4 \\ 
            $\cos$+OT, Transformer, 2 layer, 8 heads  & 44.1 & 74.8 &84.1 & 31.7 & 62.7 & 73.5 &370.9 \\
            \midrule
            PFAN & 66 & 89.6 & 94.3 & 49.6 & 77 & 84.2 & 460.7 \\
            PFAN + OT & 67.1 & 89.2 & 94.3 & 50 & 78 & 85.7 & 464.3\\
            SCAN & 46.4 & 77.4 & 87.2 & 34.4 & 63.7 & 75.7 & 384.8 \\
            SCAN + OT & 50.1 & 80.1 & 89.3 & 37.9 & 66.9 & 78.2 & 402.5 \\ 
            \bottomrule
        \end{tabular*}
    \end{center}
    % \vspace{-5mm}
\end{table*}


==> table/SM_vqa.tex <==
\begin{table}[h!]\small
    \begin{center}
    \caption{%\footnotesize 
  VQA validation dataset results
    }
    %   \vspace{-3mm}
    \label{table:sm_vqa}
    \centering
      % \begin{tabular}{lccccccc}
    %   \begin{tabular}{1.\textwidth}{@{\extracolsep{\fill}}lccc}
        \begin{tabular}{lc}
           \toprule
          %  \noalign{\smallskip}
        %    & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{}\\
          Method & VQA-score\\
          % \noalign{\smallskip}
          \toprule
          % \noalign{\smallskip}
          % & \multicolumn{7}{c}{Flickr30K} \\ 
          % \hline
          % \noalign{\smallskip}
          BAN~\cite{kim2018bilinear} & 66.06   \\
          Ours & 66.20  \\
        %   OT\_S & 25.54 & 58.05 & 69.62 \\
            \bottomrule
      \end{tabular}
  
      \vspace{-8mm}
    \end{center}
  \end{table}

==> table/ablation_PFAN.tex <==
\begin{table*}[h!] \small
    \begin{center}
    \caption{Ablation study on Flickr30K: Adding OT to existing model}
    \label{table:transformer}
    \centering
    % \begin{tabular}{lccccccc}
        \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
            \hline\noalign{\smallskip}
             & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{} \\
            Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & Rsum\\
            \noalign{\smallskip}
            \hline
            \noalign{\smallskip}
            PFAN & 66 & 89.6 & 94.3 & 49.6 & 77 & 84.2 & 460.7 \\
            PFAN + OT & 67.1 & 89.2 & 94.3 & 50 & 78 & 85.7 & 464.3

            \hline
        \end{tabular*}
    \end{center}
    % \vspace{-3mm}
\end{table*}

==> table/ablation_flickr_ad.tex <==
\begin{table*}[h!]% \small
    \begin{center}
    
    \label{table:adaptive}
    \centering
    % \begin{tabular}{lccccccc}
        \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
            \hline\noalign{\smallskip}
             & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{} \\
            Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & Rsum\\
            \noalign{\smallskip}
            \hline
            \noalign{\smallskip}
            $\cos$ + OT, fixed & 67.4 & 90.3 & 94.9 & 48.2 & 76.7 & {84.8} &462.3 \\ 
            $\cos$ + OT, adaptive & 64.8 & 88.3 &94.5 & 45.9 & 74.5 & 83.5 &451.5 \\
            \hline
        \end{tabular*}
        \caption{Ablation study in terms of Recall@$K$(R@$K$) on Flickr30K: adaptive number of regions versus fix number of regions.}
    \end{center}
\end{table*}

==> table/ablation_flickr_re.tex <==
\begin{table*}[h!] \small
    \begin{center}
    
    \label{table:flickr30k_effect_OT}
    \centering
    % \begin{tabular}{lccccccc}
        \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
            \hline\noalign{\smallskip}
             & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{} \\
            Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & Rsum\\
            \noalign{\smallskip}
            \hline
            \noalign{\smallskip}
            $\cos$, $\eta$=0.15  & 63.8 & 88.1 & 94.2 & 50.0 & 77.0 & 84.7 & 457.5 \\ 
            $\cos$ + OT, $\eta$=0.15, $\lambda$=2 & 67.4 & 90.3 & 94.9 & 48.2 & 76.7 & {84.8} &462.3 \\ 
            \hline
            $\cos$, $\eta$=0.12  & 63.1 &89.5 & 94.3 & {50.5} & 77.1 & 84.7&459.2 \\ 
            $\cos$ + OT, $\eta$=0.12, $\lambda$=2 & {69.3} & {91.0} &{95.7} & 48.4 & {77.2} & 84.7 &{466.3} \\ %OT \\
            \hline
        \end{tabular*}
        \caption{Ablation study on Flickr30K: effectiveness of OT}
    \end{center}
\end{table*}

==> table/ablation_flickr_trans.tex <==
\begin{table*}[h!] \small
    \begin{center}
    \caption{Ablation study on Flickr30K: effectiveness of network architecture}
    \label{table:transformer}
    \centering
    % \begin{tabular}{lccccccc}
        \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
            \hline\noalign{\smallskip}
             & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{} \\
            Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & Rsum\\
            \noalign{\smallskip}
            \hline
            \noalign{\smallskip}
            $\cos$+OT, bi-GRU &{67.9} &{91.0} &{94.9} &{49.8} &{77.5} &{85.2} &{466.3}\\
            $\cos$+OT, Transformer, 1 layer, 8 heads & 57.8 & 86.8 & 93.1 & 46.4 & 74.4 & {82.9} &441.4 \\ 
            $\cos$, Transformer, 2 layer, 8 heads  & 54.9 & 85.4 &91.1 & 41.2 & 70.7 & 79.8 &423.1 \\
            \hline
        \end{tabular*}
    \end{center}
    % \vspace{-3mm}
\end{table*}

==> table/coco_5folds.tex <==
\begin{table*}[h!]%\small
  \begin{center}
  \caption{Comparison of the cross-domain matching results in terms of Recall@$K$(R@$K$) on MS-COCO: results of 1k test set.}
  \label{table:mscoco_5folds}
  \centering
    % \begin{tabular}{lccccccc}
    \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
         \toprule\noalign{\smallskip}
         & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{}\\
        Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 &Rsum\\
        \noalign{\smallskip}
        \hline
        \noalign{\smallskip}
        % \hline
        % \hline
        DVSA (R-CNN, AlexNet) \cite{karpathy2015deep} & 38.4 & 69.9 & 80.5 & 27.4 & 60.2 & 74.8 & 351.2 \\ 
        HM-LSTM (R-CNN, AlexNet) \cite{niu2017hierarchical} & 43.9 & -- & 87.8 & 36.1 & -- & 86.7 & --\\ 
        Order-embeddings (VGG) \cite{vendrov2015order} & 46.7 & -- & 88.9 & 37.9 & -- & 85.9 & -- \\ 
        % DSPE (VGG) \cite{wang2016learning} & 50.1 & 79.7 & 89.2 & 39.6 & 75.2 & 86.9 \\ 
        SM-LSTM (VGG) \cite{huang2017instance} & 53.2 & 83.1 & 91.5 & 40.7 & 75.8 & 87.4 & 431.7\\ 
        2WayNet (VGG) \cite{eisenschtat2017linking} & 55.8 & 75.2 & -- & 39.7 & 63.3 & --  & --\\ 
        VSE++ (ResNet) \cite{VSE} & 64.6 & -- & 95.7 & 52.0 & -- & 92.0 & --\\ 
        DPC (ResNet) \cite{zheng2017dual} & 65.6 & 89.8 & 95.5 & 47.1 & 79.9 & 90.0 & 467.9\\ 
        GXN (ResNet) \cite{gu2018look} & 68.5 & -- & 97.9 & 56.6 & -- & 94.5 & --\\ 
        SCO (ResNet) \cite{huang2018learning} & 69.9 & 92.9 & 97.5 & 56.7 & 87.5 & -- & --\\
        SCAN t-i LSE ($\lambda_1=9,\lambda_2=6$)  & 67.5 & 92.9 & 97.6 & 53.0 & 85.4 & 92.9 & 489.3\\ 
        SCAN t-i AVG ($\lambda_1=9$) & 70.9 & 94.5 & 97.8 & 56.4 & 87.0 & 93.9  &500.5\\ 
        SCAN i-t LSE ($\lambda_1=4,\lambda_2=20$) & 68.4 & 93.9 & 98.0 & 54.8 & 86.1 & 93.3 & 494.5 \\ 
        SCAN i-t AVG ($\lambda_1=4$) & 69.2 & 93.2 & 97.5 & 54.4 & 86.0 & 93.6 &493.9\\ 
        SCAN t-i LSE + i-t AVG & {72.7} & {94.8} & {98.4} & {58.8} & {88.4} & {94.8} & 507.9 \\ 
        % \hline
        \textbf{Ours (Faster R-CNN, ResNet)} :\\
        $\cos$ + OT (single model, $\lambda$=0.1) &{66.6} &{92.3} &{97.0} &{57.9} &{87.1} &{93.9} &{494.8}\\
        $\cos$ + OT (single model, $\lambda$=0.05) &{66.8} &{92.3} &{97.1} &{57.9} &{87.0} &{93.9} &{495}\\
        % Dot + OT (single model, m=0.15) &{67.4} &{90.3} &{94.9} &{48.2} &{76.7} &{84.8} &{462.3}\\
        % Dot + OT (single model, m=0.12) &\textbf{69.3} &{91.0} &{95.7} &{48.4} &{77.2} &{84.7} &{466.3}\\
        % Dot + OT (ensembled model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        % \hline
        \bottomrule
        % & \multicolumn{7}{c}{5K Test Images} \\ 
        % \hline
        % \hline
        % Order-embeddings (VGG) \cite{vendrov2015order} & 23.3 & -- & 84.7 & 31.7 & -- & 74.6 & -- \\ 
        % VSE++ (ResNet) \cite{VSE} & 41.3 & -- & 81.2 & 30.3 & -- & 72.4 & -- \\ 
        % DPC (ResNet) \cite{zheng2017dual} & 41.2 & 70.5 & 81.1 & 25.3 & 53.4 & 66.4 & 337.9\\ 
        % GXN (ResNet) \cite{gu2018look} & 42.0 & -- & 84.7 & 31.7 & -- & 74.6 & -- \\ 
        % SCO (ResNet) \cite{huang2018learning} & 42.8 & 72.3 & 83.0 & 33.1 & 62.9 & 75.5 & 369.6 \\ 
        % SCAN i-t LSE & 46.4 & 77.4 & 87.2 & 34.4 & 63.7 & 75.7 & 384.8 \\ 
        % SCAN t-i AVG + i-t LSE & {50.4} & {82.2} & {90.0} & {38.6} & {69.3} & {80.4} & 410.9 \\ 
        % \hline
        % Ours (Faster R-CNN, ResNet) :\\
        % $\cos$ + OT ($\eta$=0.05, $\lambda$=0.1) &{50.2} &{80.1} &{89.5} &{37.9} &{66.8} &{78.1} &{402.6}\\
        % $\cos$ + OT ($\eta$=0.05, $\lambda$=0.05) &{49.9} &{81.4} &{89.8} &{37.7} &{66.7} &{78.1} &{403.6}\\
        % $\cos$ + OT (Ensemble) &\textbf{52.1} &\textbf{82.4} &\textbf{90.7} &\textbf{39.1} &{68.2} &{79.2} &\textbf{411.7}\\
        % % Dot + OT (single model, m=0.12) &\textbf{69.3} &{91.0} &{95.7} &{48.4} &{77.2} &{84.7} &{466.3}\\
        % % Dot + OT (ensembled model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        % \hline
    \end{tabular*}

  \end{center}
\end{table*}

==> table/coco_re.tex <==
\begin{table*}[h!]%\small
  \begin{center}
  \caption{Comparison of the cross-modal matching results in terms of Recall@$K$(R@$K$) on MS-COCO.}
  \label{table:mscoco}
  \centering
    % \begin{tabular}{lccccccc}
    \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
         \hline\noalign{\smallskip}
         & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{}\\
        Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 &Rsum\\
        \noalign{\smallskip}
        \hline
        \noalign{\smallskip}
        % & \multicolumn{7}{c}{1K Test Images} \\ 
        % \hline
        % \hline
        % DVSA (R-CNN, AlexNet) \cite{karpathy2015deep} & 38.4 & 69.9 & 80.5 & 27.4 & 60.2 & 74.8 \\ 
        % HM-LSTM (R-CNN, AlexNet) \cite{niu2017hierarchical} & 43.9 & -- & 87.8 & 36.1 & -- & 86.7 \\ 
        % Order-embeddings (VGG) \cite{vendrov2015order} & 46.7 & -- & 88.9 & 37.9 & -- & 85.9 \\ 
        % % DSPE (VGG) \cite{wang2016learning} & 50.1 & 79.7 & 89.2 & 39.6 & 75.2 & 86.9 \\ 
        % SM-LSTM (VGG) \cite{huang2017instance} & 53.2 & 83.1 & 91.5 & 40.7 & 75.8 & 87.4 \\ 
        % 2WayNet (VGG) \cite{eisenschtat2017linking} & 55.8 & 75.2 & -- & 39.7 & 63.3 & -- \\ 
        % VSE++ (ResNet) \cite{VSE} & 64.6 & -- & 95.7 & 52.0 & -- & 92.0 \\ 
        % DPC (ResNet) \cite{zheng2017dual} & 65.6 & 89.8 & 95.5 & 47.1 & 79.9 & 90.0 \\ 
        % GXN (ResNet) \cite{gu2018look} & 68.5 & -- & 97.9 & 56.6 & -- & 94.5 \\ 
        % SCO (ResNet) \cite{huang2018learning} & 69.9 & 92.9 & 97.5 & 56.7 & 87.5 & --\\
        % SCAN t-i LSE ($\lambda_1=9,\lambda_2=6$)  & 67.5 & 92.9 & 97.6 & 53.0 & 85.4 & 92.9 \\ 
        % SCAN t-i AVG ($\lambda_1=9$) & 70.9 & 94.5 & 97.8 & 56.4 & 87.0 & 93.9  \\ 
        % SCAN i-t LSE ($\lambda_1=4,\lambda_2=20$) & 68.4 & 93.9 & 98.0 & 54.8 & 86.1 & 93.3 & 494.5 \\ 
        % SCAN i-t AVG ($\lambda_1=4$) & 69.2 & 93.2 & 97.5 & 54.4 & 86.0 & 93.6 \\ 
        % SCAN t-i LSE + i-t AVG & {72.7} & {94.8} & {98.4} & {58.8} & {88.4} & {94.8} & 507.9 \\ 
        % \hline
        % Ours (Faster R-CNN, ResNet) :\\
        % $\cos$ + OT (single model, $\lambda$=0.1) &{66.6} &{92.3} &{97.0} &{57.9} &{87.1} &{93.9} &{494.8}\\
        % $\cos$ + OT (single model, $\lambda$=0.05) &{66.8} &{92.3} &{97.1} &{57.9} &{87.0} &{93.9} &{495}\\
        % % Dot + OT (single model, m=0.15) &{67.4} &{90.3} &{94.9} &{48.2} &{76.7} &{84.8} &{462.3}\\
        % % Dot + OT (single model, m=0.12) &\textbf{69.3} &{91.0} &{95.7} &{48.4} &{77.2} &{84.7} &{466.3}\\
        % % Dot + OT (ensembled model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        % \hline
        % & \multicolumn{7}{c}{5K Test Images} \\ 
        % \hline
        % \hline
        Order-embeddings (VGG) \cite{vendrov2015order} & 23.3 & -- & 84.7 & 31.7 & -- & 74.6 & -- \\ 
        VSE++ (ResNet) \cite{VSE} & 41.3 & -- & 81.2 & 30.3 & -- & 72.4 & -- \\ 
        DPC (ResNet) \cite{zheng2017dual} & 41.2 & 70.5 & 81.1 & 25.3 & 53.4 & 66.4 & 337.9\\ 
        GXN (ResNet) \cite{gu2018look} & 42.0 & -- & 84.7 & 31.7 & -- & 74.6 & -- \\ 
        SCO (ResNet) \cite{huang2018learning} & 42.8 & 72.3 & 83.0 & 33.1 & 62.9 & 75.5 & 369.6 \\ 
        SCAN i-t LSE & 46.4 & 77.4 & 87.2 & 34.4 & 63.7 & 75.7 & 384.8 \\ 
        SCAN t-i AVG + i-t LSE & {50.4} & {82.2} & {90.0} & {38.6} & {69.3} & {80.4} & 410.9 \\ 
        \hline
        Ours (Faster R-CNN, ResNet) :\\
        $\cos$ + OT ($\eta$=0.05, $\lambda$=0.1) &{50.2} &{80.1} &{89.5} &{37.9} &{66.8} &{78.1} &{402.6}\\
        $\cos$ + OT ($\eta$=0.05, $\lambda$=0.05) &{49.9} &{81.4} &{89.8} &{37.7} &{66.7} &{78.1} &{403.6}\\
        $\cos$ + OT (Ensemble) &\textbf{52.1} &\textbf{82.4} &\textbf{90.7} &\textbf{39.1} &{68.2} &{79.2} &\textbf{411.7}\\
        % Dot + OT (single model, m=0.12) &\textbf{69.3} &{91.0} &{95.7} &{48.4} &{77.2} &{84.7} &{466.3}\\
        % Dot + OT (ensembled model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        \hline
    \end{tabular*}
  \end{center}
\end{table*}

==> table/flickr_re.tex <==
\begin{table}[h!] \small
\begin{center}
\caption{Comparison of the cross-modal matching results in terms of Recall@$K$(R@$K$) on Flickr30K.}
\label{table:flickr30k}
  \centering
    % \begin{tabular}{lccccccc}
    \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
        \hline\noalign{\smallskip}
         & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{} \\
        Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & Rsum\\
        \noalign{\smallskip}
        \hline
        \noalign{\smallskip}
        DVSA (R-CNN, AlexNet) \cite{karpathy2015deep} & 22.2 & 48.2 & 61.4 & 15.2 & 37.7 & 50.5 & 235.2\\ 
        HM-LSTM (R-CNN, AlexNet) \cite{niu2017hierarchical} & 38.1 & -- & 76.5 & 27.7 & -- & 68.8 & --\\ 
        % DSPE (VGG) \cite{wang2016learning} & 40.3 & 68.9 & 79.9 & 29.7 & 60.1 & 72.1 \\ 
        2WayNet (VGG) \cite{eisenschtat2017linking} & 49.8 & 67.5 & -- & 36.0 & 55.6 & -- & --\\ 
        SM-LSTM (VGG) \cite{huang2017instance} & 42.5 & 71.9 & 81.5 & 30.2 & 60.4 & 72.3 & 358.8\\ 
        VSE++ (ResNet) \cite{VSE} & 52.9 & -- & 87.2 & 39.6 & -- & 79.5 & -- \\ 
        DPC (ResNet) \cite{zheng2017dual} & 55.6 & 81.9 & 89.5 & 39.1 & 69.2 & 80.9 & 416.2\\ 
        DAN (ResNet) \cite{nam2017dual} & 55.0 & 81.8 & 89.0 & 39.4 & 69.2 & 79.1 & 413.5\\ 
        SCO (ResNet) \cite{huang2018learning} & 55.5 & 82.0 & 89.3 & 41.1 & 70.5 & 80.1 & 418.5\\ 
        % SCAN t-i LSE ($\lambda_1=9,\lambda_2=6$)  & 61.1 & 85.4 & 91.5 & 43.3 & 71.9 & 80.9  \\ 
        % SCAN (Faster R-CNN, ResNet) t-i AVG ($\lambda_1=9$)  & 61.8 & 87.5 & 93.7 & 45.8 & 74.4 & 83.0 &446.2 \\ 
        % SCAN i-t LSE ($\lambda_1=4,\lambda_2=5$)   & 67.7 & 88.9 & 94.0 & 44.0 & 74.2 & 82.6 &452.2 \\ 
         SCAN (Faster R-CNN, ResNet) \cite{SCAN}  & 67.7 & 88.9 & 94.0 & 44.0 & 74.2 & 82.6 &452.2 \\ 
        % SCAN i-t AVG ($\lambda_1=4$) & {67.9} & 89.0 & 94.4 & 43.9 & 74.2 & 82.8  \\ 
        SCAN (Ensemble) \cite{SCAN} & 67.4  & {90.3} & {95.8} & {48.6} & {77.7} & {85.2} &465.0 \\
        \hline
        Ours (Faster R-CNN, ResNet):\\
        $\cos$ + OT ($\eta$=0.12, $\lambda$=1.5) &{67.9} &{91.0} &{94.9} &{49.8} &{77.5} &{85.2} &{466.3}\\
        $\cos$ + OT ($\eta$=0.12, $\lambda$=2.0) &\textbf{69.3} &\textbf{91.0} &{95.7} &{48.4} &{77.2} &{84.7} &{466.3}\\
        % $\cos$ + OT (Ensemble model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        $\cos$ + OT (Ensemble model) &{69.0} &{90.7} &{95.7} &\textbf{50.1} &\textbf{78.4} &\textbf{85.6} &\textbf{469.5}\\
        \hline
    \end{tabular*}
\end{center}
\end{table}


==> table/image_caption.tex <==
\begin{table}[h!]%\small
    % \centering
\caption{%\footnotesize 
% The performance of image captioning on the testing set of MS-COCO dataset. %
Image captioning results on MS-COCO.
}
\vspace{-3mm}
\label{table:caption_results}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
Method           & CIDEr & BLEU-4 & BLUE-3 & BLEU-2 & BLEU-1 & ROUGE & METEOR \\ \hline
%DeepVS~\cite{karpathy2015deep}  &    62.5 & 45.0 & 32.1 & 23.0 & 19.5 & 66.0 \\
Soft Attention~\cite{xu2015show}  & -- & 24.3 & 34.4 & 49.2 & 70.7 & -- &23.9\\
Hard Attention~\cite{xu2015show}  &  -- & 25.0 & 35.7 & 50.4 & 71.8 & --&23.0 \\
Show \& Tell~\cite{vinyals2015show} & 85.5 & 27.7    & --    & -- & -- & --& 23.7 \\
ATT-FCN~\cite{you2016image} &    -- & 30.4 & 40.2 & 53.7 & 70.9 & -- & 24.3\\
SCN-LSTM~\cite{gan2017semantic} & 101.2 & 33.0 & 43.3 & 56.6 & 72.8 & --& 25.7\\
Adaptive Attention~\cite{lu2017knowing}  &  108.5 & 33.2 & 43.9 &  58.0 &  74.2 & --& 26.6 \\
\hline
MLE              & 106.3 & 34.3   & 45.3   & 59.3   & 75.6   & 55.2  & 26.2   \\
Ours           & 107.5 & \textbf{34.6}   &  \textbf{45.7}   &  \textbf{59.9}   &  \textbf{76.1}   &  \textbf{55.6}  &  {26.5}   \\
\bottomrule
% (MLE+OT)+(SC+OT) & \textbf{109.8} & 34.4   & \textbf{46.4}   & \textbf{61.5}   & \textbf{78.7}   & \textbf{55.9}  & \textbf{26.7}   \\ \hline
\end{tabular}}
\vspace{-2mm}
\end{table}

==> table/retrieval_ensemble.tex <==
\begin{table*}[h!]\footnotesize
  \begin{center}
  \caption{%\footnotesize 
%   Cross-domain matching results in terms of Recall@$K$ (R@K). The results in the first section is on Flickr30K. The results in the second section is on MSCOCO.
Cross-domain matching results of ensembled model with Recall@$K$ (R@K). Upper panel: Flickr30K, lower panel: MSCOCO. 
  }
    % \vspace{-3mm}
  \label{table:retrieval_ensemble}
  \centering
    % \begin{tabular}{lccccccc}
    \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
         \toprule
        %  \noalign{\smallskip}
         & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{}\\
        Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 &Rsum\\
        % \noalign{\smallskip}
        \toprule
         SCAN (Faster R-CNN, ResNet) \cite{SCAN}  & 67.7 & 88.9 & 94.0 & 44.0 & 74.2 & 82.6 &452.2 \\ 
        % SCAN i-t AVG ($\lambda_1=4$) & {67.9} & 89.0 & 94.4 & 43.9 & 74.2 & 82.8  \\ 
        SCAN (Ensemble) \cite{SCAN} & 67.4  & {90.3} & {95.8} & {48.6} & {77.7} & {85.2} &465.0 \\
        % \hline
        BFAN (Ensemble)\cite{liu2019focus} & 68.1 & 91.4 & - & 50.8 & 78.4 & - & - \\
        PFAN (Ensemble)\cite{wang2019position} & 70.0 & 91.8 & 95 & 50.4 & 78.7 & 86.1 & 472 \\
        VSRN (Ensemble, rerun) \cite{li2019visual} & 69.3 & 91.1 & 95.7 & 52.2 & 80 & 87.5 & 475.8 \\
        VSRN (Ensemble, paper) \cite{li2019visual} & 71.3 & 90.6 & 96.0 & 54.7 & 81.8 & 88.2 & 482.6 \\
        \textbf{Ours (Faster R-CNN, ResNet)}:\\
        % $\cos$ + OT (Ensemble model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        $\cos$ + OT (Ensemble) &{70.3} &\textbf{91.5} &\textbf{96.0} &{52.2} &{79.4} &{87.1} &{476.4}\\
        % \hline
        % \hline
        \hline
        \noalign{\smallskip}

        SCAN (Faster R-CNN, ResNet)\cite{SCAN} & 46.4 & 77.4 & 87.2 & 34.4 & 63.7 & 75.7 & 384.8 \\ 
        SCAN (Ensemble)\cite{SCAN} & {50.4} & {82.2} & {90.0} & {38.6} & {69.3} & {80.4} & 410.9 \\ 
        VSRN (Ensemble, rerun)\cite{li2019visual} & 51.7 & 80.9 & 89.7 & 40.1 & 70.6 & 81.2 & 414.2 \\
        VSRN (Ensemble, paper)\cite{li2019visual} & 53.0 & 81.1 & 89.4 & 40.5 & 70.6 & 81.1 & 414.2 \\
        % \hline
        \textbf{Ours (Faster R-CNN, ResNet)}:\\
        $\cos$ + OT (Ensemble) &{52.1} &\textbf{82.4} &\textbf{90.7} &{39.1} &{68.2} &{79.2} &{411.7}\\
        % Dot + OT (single model, m=0.12) &\textbf{69.3} &{91.0} &{95.7} &{48.4} &{77.2} &{84.7} &{466.3}\\
        % Dot + OT (ensembled model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        \bottomrule
    \end{tabular*}

    % \vspace{-5mm}
  \end{center}
\end{table*}
